HammerBench: Fine-Grained Function-Calling Evaluation in Real Mobile Device Scenarios

Evaluating the performance of LLMs in multi-turn human-agent interactions presents significant challenges, particularly due to the complexity and variability of user behavior. In this paper, we introduce HammerBench, a novel benchmark framework for assessing LLMs' function-calling capabilities in real-world, multi-turn dialogues. HammerBench simulates diverse mobile assistant use cases, incorporating imperfect instructions, dynamic question-answer trajectories, intent and argument shifts, and the indirect use of external information through pronouns. To construct this benchmark, we curate a comprehensive dataset derived from popular mobile app functionalities and anonymized user logs, complemented by a cost-effective data generation pipeline leveraging open-source models. HammerBench is further augmented with fine-grained interaction snapshots and metrics, enabling detailed evaluation of function-calling performance across individual conversational turns. We demonstrate the effectiveness of HammerBench by evaluating several leading LLMs and uncovering key performance trends. Our experiments reveal that different types of parameter name errors are a significant source of failure across different interaction scenarios, highlighting critical areas for further improvement in LLM robustness for mobile assistant applications.

==> src/4_HammerBench.tex <==

In this section, we outline the methodology used to generate various datasets. All datasets are constructed using open-source LLMs, including Qwen2.5-72B-Instruct-GPTQ-Int4 and Llama-3.1-70B-Instruct-GPTQ-Int4.

\subsection{Test Data Construction}

The construction of the dataset in \hb follows a systematic approach, beginning with the collection of the toolset and followed by the automatic generation, validation, and manual refinement of the dataset. The overall process refers to \Cref{fig:generation pipline}.

\textbf{Tool collection and API Generation:} Toolset in \hb is collected for mobile users, focusing on functionalities commonly found in OPPO App Store applications. We begin by identifying highly downloaded apps, clustering them into 60 functional categories based on expert opinions. Descriptive prompts (see \Cref{appx:Tool Generation}) are created for each category, and APIs are generated using LLMs. Given the limitations of simple prompts, the generation process is broken into stages: generating function names, descriptions, parameters, and returns. Human oversight is incorporated at each stage to ensure usability and avoid overly complex parameters. Redundancy is minimized by ensuring distinct tool functionalities within each category.

\textbf{Validation and Refinement:} Each generated API is then subjected to a thorough manual review and refinement process to ensure its quality and applicability. This process results in the final selection of 1,063 APIs. This process is guided by two core principles: completeness and rationality. Completeness ensures that the APIs within each functional category adequately cover all typical usage scenarios, thereby ensuring that they represent the full range of possible interactions within that category. Rationality, on the other hand, requires that the definition, input, and output of each API are both clear and concise, avoiding unnecessary complexity while maintaining operational integrity. To facilitate the generation of function-calling instances, we apply the self-instruct method (\citealp{wang-etal-2023-self-instruct}) to create function-calling instances. This process yields three types of instructions: (1) perfect instructions, which correspond to complete function calls with all required parameters; (2) imperfect instructions, where one or more key arguments are missing; and (3) function-irrelevant instructions, which trigger a rejection signal when no appropriate function can be called. The refinement process ensures that each API is both functional and user-friendly, enabling accurate and efficient evaluation within the benchmark framework.

\begin{figure*}[htb]
  \centering
  % \fbox{\rule[-.5cm]{4cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \includegraphics[width=1\textwidth]{picture/generation_pipline}
  \caption{\hb consists of following process: toolset construction, data generation, external knowledge generation and check module, and finally obtains generated datasets. Besides, the external individual information part serves as an auxiliary module that converts the query-label pairs generated from the three stages into instances with pronouns. Blocks with GPT icons indicate the integration of LLMs, while the orange block represents the verification module. Green blocks are used to denote the various data types corresponding to each phase.}
  \label{fig:generation pipline}
\end{figure*}

\subsubsection{Multi-Turn Interactions for Imperfect Instructions}\label{sec:imperfect}
Given that 76\% of the queries in user logs contain fewer than 10 tokens, we devised a methodology to generate datasets that reflect these typical query lengths. For each API, we first prompt large language models (LLMs) to identify the parameters most frequently used in daily applications, as illustrated in \Cref{fig:generation pipline}. The corresponding prompt for parameter selection is provided in \Cref{appx:Parameters Selection}. Subsequently, LLMs are constrained to generate instructions that incorporate these selected parameters (see \Cref{appx:Query Generation}). If any parameters are missing or extraneous parameters are included, the model is instructed to regenerate the query until it adheres to the preset parameter list.

Through this process, we obtain imperfect instances that pass format verification. However, it is observed that hallucinations are prevalent in these instances. To mitigate this, we introduce a semantic validation step inspired by prior work (\citealp{li-etal-2024-one}). Specifically, for each generated instance, we assess whether the function call generated by the LLM remains consistent when the instruction is presented in both zero-shot and one-shot in-context learning settings. Consistency is evaluated using two metrics: (1) Rouge-L, with a pre-defined threshold, and (2) semantic alignment, which is measured by re-evaluating the function call with the LLM. The rationale behind this semantic checking process is that instructions that are correctly processed in a zero-shot scenario are considered more reliable and less prone to hallucinations. These instances are thus re-validated, first through zero-shot and then through one-shot learning.

Once these instances are selected, they undergo manual inspection to ensure overall quality. A sampling review is conducted to further assess the integrity of the generated function calls. Ultimately, this process yields 3,240 imperfect instances, which serve as the foundation for constructing basic multi-turn function-calling scenarios, as detailed in the following sections.

\begin{figure*}[htb]
  \centering
  \includegraphics[width=1\textwidth]{picture/examples_of_dataset}
  \caption{Examples of four types of test cases in \hb: 1) Diverse Q\&A trajectories are generated by randomly merging user-agent interactions; 2) Intent shifts: agent should terminate the current session when users change their intent during the Q\&A process; 3) Argument shifts: three cases of changing slot values during the interactions; 4) External individual information: users answer with pronouns instead of exact external information, which are frequently encountered in real-world interactions.}
  \label{fig:examples of dataset}
\end{figure*}

\subsubsection{Diverse Question-answer Trajectories}\label{sec:qa}

Building on the imperfect instructions outlined in the previous section, we extend these instances to create multi-turn function-calling dialogues that involve interactive slot-filling. To evaluate the model's ability to handle varying conversational flows, we design four distinct types of question-and-answer trajectories:
\begin{itemize}
    \item \textbf{Single-Question-Single-Answer:} In this trajectory, the model queries a single argument, and the user responds with a corresponding single value. This basic structure ensures that the model can accurately elicit a single piece of information.
    \item \textbf{Multi-Question-Multi-Answer:} In this trajectory, the model queries a single argument, and the user responds with a corresponding single value. This basic structure ensures that the model can accurately elicit a single piece of information.
    \item \textbf{Single-Question-Multi-Answer:} In this scenario, the model inquires about a single argument, but the user provides answers that correspond to multiple arguments. This trajectory challenges the model's ability to handle more nuanced user responses and manage multiple interpretations of a query.
    \item \textbf{Multi-Question-Single-Answer:} The model presents multiple questions, yet the user answers only one. This scenario is designed to test the model's ability to handle incomplete information and adapt to user responses that do not follow the expected trajectory.
\end{itemize}

To construct these trajectories, we first generate single-question-single-answer instances using the prompts provided in \Cref{appx:Multi-turn Prompt}. These instances undergo the semantic checking and human review processes discussed in \Cref{sec:imperfect}. Subsequently, the remaining trajectories are derived by combining the questions and/or answers from the single-question-single-answer dataset. Specifically, we randomly merge questions posed by the model and answers provided by the user to form the different dialogue structures. This approach results in a diverse range of multi-turn interaction patterns, ultimately producing 2,310 distinct instances for evaluation.

\subsubsection{Intent and Argument Shifts}

In real-world interactions, users often exhibit abrupt shifts in their intentions or modify their slot values for various reasons. For instance, if a tool requires excessive parameter input, users may find the process cumbersome and opt for a different tool, or they may unexpectedly change their goal midway through the interaction. In this section, we aim to evaluate whether the model can recognize such intent shifts and appropriately respond with a rejection signal, thereby terminating the conversation.

To build the dataset for intent shifts, we begin with instances derived from the \textit{Single-Question-Single-Answer} trajectories. Specifically, we randomly select a user input within a dialogue and replace it with an arbitrary single-turn function call instruction pertaining to a different API, as shown in \Cref{fig:examples of dataset}. This randomization process enables the creation of 1,098 instances that simulate sudden shifts in user intent. Additionally, we consider two types of argument shifts that challenge the model's ability to handle evolving user input: slot overriding and repurposing of the API after a function call.

For slot overriding, users may introduce multiple values for the same parameter across a dialogue, but only the most recent value is required for the function call. This shift can be particularly challenging for models, as they must accurately recognize and apply the most up-to-date argument. To generate these instances, we modify several \textit{Single-Question-Single-Answer} dialogues, either by inserting new turns where users explicitly request to override a previous argument or by appending an override request at the end of an existing user input. This process yields 1,462 instances involving slot overriding.

In the case of repurposing the API, users may alter certain parameters of an already executed function call while retaining the original values for others. This shift tests the model’s flexibility in reusing prior function calls while adapting to new input values. To construct these instances, we insert a new user input turn after a function call, introducing updated parameter values while preserving the existing ones. In total, 1,066 instances involving repurposing are generated.

\subsubsection{References to External Individual Data}
In user interactions with AI assistants, it is common for users to reference information through pronouns, rather than providing specific values directly. This is particularly true when users seek to retrieve or reference external data not explicitly stated within the conversation. To evaluate models' abilities in Anaphora Resolution, we propose a novel approach for generating datasets that incorporate references to external individual data, as depicted in the right-hand section of \Cref{fig:generation pipline}. These references can be drawn from any single-turn or multi-turn function call instance, with no limitation on the method of external data acquisition, such as retrieval tools or other resources.

The dataset construction begins by selecting nine distinct information entities commonly referenced in such scenarios, including human names, company names, product identifiers, license plate numbers, ID numbers, time, location, songs and singers, and five specific applications (SMS, Email, Instant Messaging, Social Media, and Notebook). These entities serve as external sources that carry the precise values for these references. For each instance, we use LLMs to identify whether any of the argument values from previous instances correspond to these entities. We then reserve those instances that contain such references for further processing.

Next, for each reserved instance, one argument—corresponding to an identified entity—is selected for replacement with a pronoun. LLMs are employed to simulate a text message, which contains the argument value and links it to one of the external sources, as illustrated in the right portion of \Cref{fig:generation pipline}. The instruction is then rewritten to include the pronoun referring to the external entity. This results in the creation of a new instance that reflects the reference to external individual data.

Prior to finalization, all instances undergo a semantic validation and manual inspection process similar to the previous steps. This ensures that the generated queries are both contextually accurate and free from contradictions. Through this approach, we generate 1,175 single-turn and 487 multi-turn instances that incorporate references to external individual data. All relevant prompts used in this process are detailed in \Cref{appx:external individual information Prompt}.

\subsubsection{Function Calling Snapshots}
\muning{Remember to improve the coherence here.}
We conducted a comparative experiment to validate the reliability of breaking down conversations into snapshots. To eliminate the potential influence of post-training, we fine-tuned Qwen2.5-7B with two distinct training paradigms: Learning to Ask and Function Calling Snapshots. Both models were evaluated on the same 100 out-of-distribution (OOD) conversations, where human interaction and manual annotation were employed for scoring.

The \textbf{Leaning to Ask} paradigm involves fine-tuning LLMs to generate appropriate questions for missing argument values directly at each turn, and subsequently output the function call after all parameter values are completed. In contrast, the \textbf{Function Calling Snapshots} paradigm fine-tunes LLMs to generate function calls at each conversational turn, while the questions themselves are generated using a rule-based approach. The results, as shown in \Cref{table:snapshot}, indicate that training on function calling snapshots yields a 16\% higher success rate compared to the Leaning to Ask approach. Based on these findings, we proceed to evaluate function-calling snapshots at each turn in the conversation. Three distinct types of snapshots were chosen for this evaluation: (1) the final turn of the conversation, (2) the snapshot at the moment when the user changes slot values, and (3) every snapshot throughout the conversation.

\begin{table}[htb]
\centering
\begin{tabular}{ll}
\toprule
Training Paradigm  & SR \\
\midrule
Learning to Ask    & 68\%  \\
Function Calling Snapshots & 84\%  \\
\bottomrule
\end{tabular}
\caption{Comparison between Learning to Ask and Function Calling Snapshots paradigms.}
\label{table:snapshot}
\end{table}

\subsection{Fine-Grained Evaluation Metrics}
To assess the performance of function-calling across various conversational snapshots, we employ several key evaluation metrics, as outlined below. These metrics, when combined, provide a comprehensive overview of the model's performance throughout the entire conversation. Similar to the methodology used in NoisyToolBench (\citealp{NoisyToolBench}), we prompt Llama-3.1-70B-Instruct-GPTQ-Int4 to determine the correctness of each snapshot prediction. The metrics are as follows:

\begin{itemize}

\item \textbf{Function Name Accuracy (Func Acc)} evaluates the accuracy of the predicted function names within function-calling samples.

\item \textbf{Function-Irrelevant Accuracy (Irrelevant)} quantifies the proportion of function-calling samples where the model correctly identifies all irrelevant functions. A high Irrelevant score reflects the model's ability to detect and exclude irrelevant information from the function call.

\item \textbf{Parameter Names Hallucination and Missing Rate (PHR/MR):} In scenarios where the function names are predicted correctly, PHR represents the proportion of samples where the model predicted parameter names not provided in the definition, while PMR indicates the proportion of samples where the model fails to predict all parameter names in ground truth. These metrics help assess the accuracy and completeness of parameter name predictions.

\item \textbf{Agrs Acc} Given that both the function name and parameter names are correct, Args Acc will be True if all parameter values are correctly filled, measuring the average accuracy of function calling across considered snapshots. Args Acc provides a detailed assessment of the model's ability to handle both the function name and its parameters simultaneously.

\item \textbf{Progress Rate (PR):} For multi-turn conversations, let $n$ denote the total number of snapshots in the conversation, and $k$ the number of snapshots that are correctly filled in from the beginning. The Progress Rate is then defined as $PR=\frac{k}{n}$, representing the proportion of correctly predicted snapshots at each stage of the conversation. This metric is designed to track the progress of function calling throughout multi-turn interactions.

\item \textbf{Success Rate (SR)} measures the proportion of dialogues in which all function-calling snapshots across the entire conversation are correct. This end-to-end metric reflects the overall accuracy of the function calls within the context of the conversation.
\end{itemize}

Together, these metrics—Func Acc, Args Acc, PHR, PMR, SR, and PR—offer a robust framework for evaluating the performance of function calling across both individual turns and multi-turn dialogues. It is important to note that, in contrast to single-turn evaluations, the success rate in multi-turn conversations takes into account the accuracy of function calling across all conversational turns, ensuring a holistic assessment of the model’s performance in dynamic, multi-turn interactions.

